Rethinking Adversarial Policies: A Generalized Attack Formulation and Provable Defense in RL

Most existing works focus on direct perturbations to the victim's state/action or the underlying transition dynamics to demonstrate the vulnerability of reinforcement learning agents to adversarial attacks. However, such direct manipulations may not be always realizable. In this paper, we consider a multi-agent setting where a well-trained victim agent $\nu$ is exploited by an attacker controlling another agent $\alpha$ with an \textit{adversarial policy}. Previous models do not account for the possibility that the attacker may only have partial control over $\alpha$ or that the attack may produce easily detectable "abnormal" behaviors. Furthermore, there is a lack of provably efficient defenses against these adversarial policies. To address these limitations, we introduce a generalized attack framework that has the flexibility to model to what extent the adversary is able to control the agent, and allows the attacker to regulate the state distribution shift and produce stealthier adversarial policies. Moreover, we offer a provably efficient defense with polynomial convergence to the most robust victim policy through adversarial training with timescale separation. This stands in sharp contrast to supervised learning, where adversarial training typically provides only \textit{empirical} defenses. Using the Robosumo competition experiments, we show that our generalized attack formulation results in much stealthier adversarial policies when maintaining the same winning rate as baselines. Additionally, our adversarial training approach yields stable learning dynamics and less exploitable victim policies.

==> 4_attack.tex <==
\section{Controllable stealthy adversarial policies}
\label{sec:controalledAA}
\textbf{Problem description.} We consider a multi-agent system with two agents, $\nu$, and $\alpha$, the interaction between which can be cooperative, competitive, or mixed. TODO: footnote The policies adopted by $\nu$ and $\alpha$ are denoted as $\hat{\pi}_\nu$ and $\hat{\pi}_\alpha$. We consider the attack model as in \cite{gleave2019adversarial, wu2021adversarial, guo2021adversarial}, where the adversarial threat is not from the perturbations of states or actions, but from some attacker which controls the agent $\alpha$, acting adversarially against agent $\nu$ by deviating from $\hat{\pi}_\alpha$ to the adversarial policy $\pi_\alpha$. Therefore, the interaction between the attacker and the victim agent $\nu$ can be modeled as a zero-sum game, although before the attacker taking control of agent $\alpha$, the two agents do not necessarily compete with each other. Correspondingly, the victim has the objective of developing a more robust policy $\pi_\nu$ instead of the original $\hat{\pi}_\nu$, preparing for the potential adversarial policies. Finally, we remark that our problem can be also extended to the system with more than two agents, where one {\it team} of agents are adversarially controlled and the other {\it team} needs to make corresponding defenses. However, such {\it two-team} problem is substantially harder than the {\it two-agent} problem \citep{kalogiannistowards} and we leave for further investigations. TODO: to generalize to multiple agents

%\fhc{Unnaturally connection between two paragraphs.}
Although such attacks can successfully exploit the victim, for many practical scenarios unlike the attacks in \cite{gleave2019adversarial, wu2021adversarial, guo2021adversarial}, the attacker could confront resistance and take only {\it partial} control of the agent $\alpha$, e.g., hijack. Furthermore, if the adversarial policy is optimized in an {\it unconstrained} way with the {\it only} goal of minimizing the performance of the victim, it could introduce perceivably weird behaviors and be easily detected by even human eyes \citep{gleave2019adversarial}, thus being less harmful.

%\cite{gleave2019adversarial} consider a different attack model in which attacks are realized through actions of an adversarial agent in the same environment as the victim.
%Although principled, the attacking formula may be too strong as the attacks may no longer be stealthy or imperceptible. 
%People may argue that once the attacks are non-stealthy, they can be easily recognized and thus no longer be harmful, especially in a setting that is meant to be cooperative.
% \fhst{To begin with, we remark that the attacking formula in} \citep{gleave2019adversarial} 
% \fhst{is too strong in the senses that such attacking scheme is not compatible with the generally accepted concept of "adversarial", which means the perturbations or attack should be imperceptible at least to humans eyes. However, the adversarial policy obtained by the framework of unconstrained attack can induce obviously weird behaviors, which could be easily detected. }


%\xyedit
With the goal of characterizing the partial control of the attacker and looking for {\it stealthier} attacks, we provide the following more generalized attack framework. We start from characterizing the stealthiness of the attack and connect it back to the partial control of the attacker.
Here, we make one essential hypothesis that humans usually detect the presence of adversarial behaviors by tracking the states of the multi-agent systems. 
%\xyedit
TODO: avoid detection

{Another possible option is to track the actions or rewards of each agent. 
However, in many practical multi-agent systems, agents are decentralized and the action or reward is private to each agent \citep{zhang2018fully} and not available to humans who hope to detect potential adversarial behaviors.}
Therefore, for the adversarial agent to hide the adversarial behaviors from being detected, we propose to control the perturbation of the system states. 
Formally, we offer our attack objective as the following optimization problem.
\begin{align}
\label{eq:obj}&\min_{\pi_{\alpha}}V_{\rho}(\hat{\pi}_{\nu}, \pi_{\alpha})\\
\label{eq:divergence}&\text{s.t.}\quad ||d_\rho^{\hat{\pi}_{\nu}, \hat{\pi}_{\alpha}} - d_\rho^{\hat{\pi}_{\nu}, \pi_{\alpha}}||_1\le \epsilon_d.
\end{align}
The objective \eqref{eq:obj} is a common attack objective \citep{gleave2019adversarial,guo2021adversarial,wu2021adversarial}, where the adversarial player $\nu$ aims to minimize the value of the victim $\alpha$. Apart from the objective, we propose further to constrain the behavior of the adversarial policy $\pi_{\alpha}$ so that the induced state visitation of $d_\rho^{\hat{\pi}_\nu, \pi_{\alpha}}$ stays close to the original $d_\rho^{\hat{\pi}_\nu, \hat{\pi}_{\alpha}}$. 

% \xy{Motivation for constraints:

% 1. gleave paper image visual effects

% 2. actions not perceivable in some domains

% 3. illusionary attack not feasible}

However, it is generally difficult to estimate the state visitation for given policies, let alone enforce the constraints in Equation \eqref{eq:divergence}. 
Therefore, in the remaining section, we will try to find an upper bound for the discrepancy between state visitation. The key idea is to show that the distance between state visitation can be upper bounded by the distance between policies. To do so, we first define the distance between the two policies as follows
\begin{definition}[Attack Budget]\label{def:budget}
We define the attack budget as the maximum total variation distance $D_{\operatorname{TV}}^{\max}$ between two policies:
TODO: use notation $\alpha$
$
    D_{\operatorname{TV}}^{\max}(\pi||\pi^{\prime}) = \max_{s}D_{\operatorname{TV}}(\pi(\cdot|s)||\pi^{\prime}(\cdot|s)),
$
where $D_{\operatorname{TV}}(p||q) = \frac{1}{2}\sum_i |p_i-q_i|$.
\end{definition}
This definition gives a more straightforward way to control the variation of the policy at every state $s$. 
However, it is unclear how this definition relates to the total variation between state visitations. 
We answer it in \cref{theorem:1}.   
\begin{theorem}\label{theorem:1}
For two victim-attacker policy pairs $(\hat{\pi}_{\nu}, \hat{\pi}_{\alpha})$ and $(\hat{\pi}_{\nu}, \pi_{\alpha})$, where $D_{\operatorname{TV}}^{\max}(\pi_{\alpha}||\hat{\pi}_{\alpha})\le \epsilon_\pi$, the difference between the state visitation can be bounded as:
% \begin{align*}
$
    ||d_\rho^{\hat{\pi}_{\nu}, \hat{\pi}_{\alpha}}-d_\rho^{\hat{\pi}_{\nu}, \pi_{\alpha}}||_{1}\le \frac{2\gamma\epsilon_\pi}{1-\gamma}.
$ Furthermore, we have the value difference bounded as: $
    |V_{\rho}(\hat{\pi}_\nu, \hat{\pi}_\alpha) - V_{\rho}(\hat{\pi}_\nu, \pi_\alpha)|\le\frac{2\epsilon_\pi}{(1-\gamma)^2}.
$

% \end{align*}
\end{theorem}
% \begin{proof}
% See Appendix \ref{app:1}.
% \end{proof}
% \vspace{-2mm}
TODO: another problem

This theorem shows a relationship between $D_{\operatorname{TV}}^{\max}(\pi_{\alpha}||\hat{\pi}_{\alpha})$ and $||d_\rho^{\pi_{\nu}, \pi_{\alpha}}-d_\rho^{\pi_{\nu}, \hat{\pi}_{\alpha}}||_{1}$: to control the variation of the state visitation, it {\it suffices} to control the policy variation at each state. 
%Meanwhile, with the state distribution variation controlled, we derive the following upper bound:
%\begin{proposition}\label{corr:1}
%Under the same condition of Theorem \ref{theorem:1}, the value difference holds that
%% \begin{align*}
%$
%    |V_{\rho}(\hat{\pi}_\nu, \hat{\pi}_\alpha) - V_{\rho}(\hat{\pi}_\nu, \pi_\alpha)|\le\frac{2\epsilon_\pi}{(1-\gamma)^2}.
%$
%% \end{align*}
%\end{proposition}
In addition, it suggests that the value function naturally satisfies a Lipschitz condition, where the attacker must have enough budget to achieve large performance degradation, standing in contrast with the adversarial attack in supervised learning, where small perturbations suffice to make huge changes to the final outputs. Formally, this tells us the performance drop is at most $\frac{2\epsilon_\pi}{(1-\gamma)^2}$ when the attacker has the attack budget $\epsilon_\pi$. Although these two bounds are just upper bounds and may not be tight, they still tells us that when $\gamma$ is close to $1$ meaning the game has a long effective horizon, the attacker would have more capability in degrading the victim's performance.



\paragraph{A parameterization that converts the constrained problem to unconstrained.}
% {\fhst{To enforce the more sufficient constraint}}
%\fhc{what does this sentence mean?} 
%\xlc{because what we constrain is the policy variation, an upper bound of state distribution variation as in theorem 1. Therefore, controlling the policy variation is more sufficient}
As shown in Theorem~\ref{theorem:1}, policy variation upper-bounds the state distribution variation.
Consequently, rather than directly constrain state visitation distribution, we constrain policy variation $D_{\operatorname{TV}}^{\max}(\pi_{\alpha}||\pi_{\alpha}^{\prime})$, which can be realized more efficiently.
We use the idea from \citep{kakade2002approximately} and convert the constrained problem to the unconstrained one by using the following parameterization.
\begin{definition}[$\epsilon$ coupling]
Fix $\epsilon\ge 0$. The $\epsilon$ coupled policy is constructed for each state $s\in \mathcal{S}$
\begin{align}
\label{coupling}\pi_{\alpha}(\cdot\given s)=(1-\epsilon)\hat{\pi}_{\alpha}(\cdot\given s) + \epsilon\Tilde{\pi}_\alpha(\cdot\given s),
\end{align}
where $\Tilde{\pi}_\alpha$ is what the attacker tries to optimize.  
\end{definition}

TODO: coupling cover many cases

With $\epsilon$ coupling, it is easy to verify the following proposition.
\begin{proposition}\label{tv_dis}
Fix $\epsilon\ge 0$, with $\pi_{\alpha}$ defined as Equation \eqref{coupling}, it holds for any $\Tilde{\pi}_\alpha$ that
% \begin{align*}
$
D_{\operatorname{TV}}^{\max}(\pi_{\alpha}||\hat{\pi}_{\alpha})\le \epsilon.
$
% \end{align*}
\end{proposition}
% \begin{proof}
% For simplicity, let us assume the action space is finite and discrete. For continuous case, one can simply replace the sum as integrals. Firstly, note that for any state $s$:
% \begin{align}
% &d_\rho^{\operatorname{TV}}(\pi_{\nu}(\cdot|s)||\pi_{\nu}^{\star}(\cdot|s))\\&=\frac{1}{2}\sum_{a}|\pi_{\nu}(a|s)-\pi_{\nu}^{\star}(a|s)|\\&=\frac{1}{2}\sum_{a}|(1-\lambda)\pi_{\nu}^{\star}(a|s)+\lambda\pi(\theta)(a|s)-\pi_{\nu}^{\star}(a|s)|\\&=\frac{1}{2}\lambda\sum_a|\pi(\theta)(a|s)-\pi_{\nu}^{\star}(a|s)|\\&=\lambda d_\rho^{\operatorname{TV}}(\pi(\theta)||\pi_{\nu}^{\star})\\&\le \lambda
% \end{align}
% Therefore, for $d_\rho^{\operatorname{TV}}^{\max}$, we have:
% \begin{align}
% d_\rho^{\operatorname{TV}}^{\max}(\pi_{\nu}||\pi_{\nu}^{\star})=\max_{s}d_\rho^{\operatorname{TV}}(\pi_{\nu}(\cdot|s)||\pi_{\nu}^{\star}(\cdot|s))\le \lambda
% \end{align}
% \end{proof}
%\xyedit
Therefore, the objective \eqref{eq:obj} can be replaced by the alternative objective $\min_{\Tilde{\pi}_\alpha}V_{\rho}(\hat{\pi}_{\nu}, (1-\epsilon_\pi)\hat{\pi}_{\alpha} + \epsilon_\pi \Tilde{\pi}_\alpha)$, where $\epsilon_\pi = \frac{1-\gamma}{2\gamma}\epsilon_d$ according to Theorem \ref{theorem:1} and Proposition \ref{tv_dis}.

\paragraph{Connection to stealthiness and detectability in single-agent RL.} \cite{russo2021balancing,franzmeyer2022illusionary} also considers stealthy attack but under a {\it different} setting with adversarial state or action perturbations in single-agent RL. The corresponding notion of stealthiness or detectability relies on the inconsistencies in {\it transition dynamics} when states or actions are adversarially perturbed. However, in our problem, the (global) transition dynamics $P$ will not be affected by the adversarial policy $\pi_\alpha$. Meanwhile, it is also possible to compare the {\it marginalized} transition dynamics induced by $\hat{\pi}_\alpha$ and $\pi_\alpha$ from the perspective of the victim $\nu$. Formally, we have the following proposition.
\begin{proposition}\label{prop:detection}
We define the {\it marginalized} transition dynamic of agent $\nu$ as $P^{\pi_\alpha}_\nu(s^\prime\given s, a_\nu) := \EE_{a_\alpha\sim \pi_\alpha(\cdot\given s)}[P(s^\prime\given s, a_\alpha, a_\nu)]$ for given $\pi_\alpha$. $P^{\hat{\pi}_\alpha}_\nu$ is defined similarly for the policy $\hat{\pi}_\alpha$. Then for any $s\in\cS$ and $a_\nu\in \cA_\nu$, we have
		\begin{align*}
			D_{f}\left(P^{\pi_\alpha}_\nu(\cdot \given s, a_\nu)\mid\mid P^{\hat{\pi}_\alpha}_\nu(\cdot \given s, a_\nu)\right)\le D_{f}\Big(\pi_\alpha(\cdot \given s)\mid\mid \hat{\pi}_\alpha(\cdot \given s)\Big),
		\end{align*}
	where $D_f$ is any $f$-divergence, which includes total variation distance, the attack budget we consider in Definition \ref{def:budget}.
\end{proposition}
This proposition tells us that the inconsistencies in the marginalized transition dynamics can be also upper-bounded by the variation in the policy space, thus guaranteeing low {\it detectability} considered in \cite{russo2021balancing,franzmeyer2022illusionary}. Therefore, even if the human or the detector can have access to the private actions of the agent $\nu$ and fit the corresponding marginalized transition dynamics accurately, it may not detect large discrepancies as long as the policy space variation of $\alpha$ is small.
\paragraph{Connection to action robust RL.} Interestingly, we remark that our attack formulation also generalizes the single-agent action robust RL in \cite{tessler2019action} to the multi-agent setting. Indeed, in PR-MDP (c.f. Definition 1. of \cite{tessler2019action}), the policy under attack has exactly the same formula as our Equation \eqref{coupling}, where the adversarial policy $\Tilde{\pi}_\alpha$ is only a {\it part} of the finally executed policy but the policy $\hat{\pi}_\alpha$ needs to make corresponding defense. Therefore, our formulation also generalizes the attack setting of \cite{tessler2019action} to multi-agent RL and investigates the defense for the {\it other} agent $\nu$ instead of the adversarially controlled agent $\alpha$. Furthermore, to find the most robust policy, the policy iteration scheme for PR-MDP of \cite{tessler2019action} is no longer efficient in our problem due to the lack of specific structures as in PR-MDP, since when $\epsilon_\pi = 1$, our defense problem reduces to a {\it vanilla} Markov game, where policy iteration needs to solve a max-min problem at each step. For more detailed discussions, we refer to Section 4 of \cite{tessler2019action}.

Hereafter, we will write $\Tilde{\pi}_\alpha$ as $\pi_\alpha$ for short without ambiguation and the actually deployed policy for agent $\alpha$ is $(1-\epsilon_\pi)\hat{\pi}_{\alpha} + \epsilon_\pi \pi_\alpha$. All proofs of discussions in this section can be found in Appendix \ref{sec:full_proof}. TODO: discuss the optimization





